Language Inclusion for Finite Prime Event Structures

We study the problem of language inclusion between finite, labeled prime event structures. Prime event structures are a formalism to compactly represent concurrent behavior of discrete systems. A labeled prime event structure induces a language of sequences of labels produced by the represented system. We study the problem of deciding inclusion and membership for languages encoded by finite prime event structures and provide complexity results for both problems. We provide a family of examples where prime event structures are exponentially more succinct than formalisms that do not take concurrency into account. We provide a decision algorithm for language inclusion that exploits this succinctness. Furthermore, we provide an implementation of the algorithm and an evaluation on a series of benchmarks. Finally, we demonstrate how our results can be applied to mutation-based test case generation.

==> applications.tex <==
\section{Applications}
\label{sec:applications}

Language inclusion of prime event structures is useful whenever two systems can be expressed as prime event structures. It is particularly beneficial for systems with inherent concurrency, where prime event structures are very succinct.

\subsection{Mutation-based test case generation}

Our motivation to investigate event structures and language inclusion was model-based mutation testing. 
The goal of \emph{model-based testing} (MBT) is to derive test-cases from a model of a system. 
The model may, for example, be a UML state machine and the test may be a sequence of inputs and outputs of the system. The simplest way of obtaining such test cases would be to randomly explore the state machine and record the produced input/output (IO) sequences. 
These tests can then be run against an implementation at a later point.

\emph{Model-based mutation testing} (MBMT) compares the original model to a mutated version of it. 
A mutation is a small change in the model, such as removing or adding a transition. 
Then a test case is only generated if it shows a difference between the original and the mutated model. 
This test case generation can be easily expressed using language inclusion between the two versions of the system: 
The test is exactly the word that is a member of the mutant, but not of the original.

The use of event structures is motivated by two factors. Firstly, models often use parallely running state machine that synchronize rarely. Secondly, for the test case generation we only consider the part until the input is required by the model, which is typically finite. This is motivated by the IO conformance~\cite{tretmans1996test}, which roughly-speaking allows the mutant to accept different inputs, but not to produce different outputs.

We implemented this approach and present the results in \cref{sec:experiments}.


\subsection{Other uses}

We envision numerous other applications that we did not investigate in depth. 

\paragraph*{Regression checking and version comparison}

Since many concurrent system can be concisely represented as an event structure comparison of these structures makes sense to find semantic differences between two versions of a software. This can, for example, be used to find regressions if between two versions the observable behavior of the system changed.

\paragraph*{Bounded model checking}

Model checking basically involves checking if a system exhibits the same behavior as a model. 
It differs from MBMT in that for MBMT tests are generated from the model and later run against the implementation. 
For model-checking, the implementation has to exist. 
Therefore one event system would be built from the model and one from the implementation. 
The language inclusion check can then verify that the implementation operates within the specification of the model.


